Cross-Modal Fusion Distillation for Fine-Grained Sketch-Based Image Retrieval

Representation learning for sketch-based image retrieval has mostly been tackled by learning embeddings that discard modality-specific information. As instances from different modalities can often provide complementary information describing the underlying concept, we propose a cross-attention framework for Vision Transformers (XModalViT) that fuses modality-specific information instead of discarding them. Our framework first maps paired datapoints from the individual photo and sketch modalities to fused representations that unify information from both modalities. We then decouple the input space of the aforementioned modality fusion network into independent encoders of the individual modalities via contrastive and relational cross-modal knowledge distillation. Such encoders can then be applied to downstream tasks like cross-modal retrieval. We demonstrate the expressive capacity of the learned representations by performing a wide range of experiments and achieving state-of-the-art results on three fine-grained sketch-based image retrieval benchmarks: Shoe-V2, Chair-V2 and Sketchy. Implementation is available at https://github.com/abhrac/xmodal-vit.

==> tex/06_limitations.tex <==
% \section{Negative Societal Impact}
% \label{sec:negative_societal_impact}

\section{Limitations and Negative Societal Impact}
\label{sec:limitations}
%The underlying technique of our proposed XModalViT model for fine-grained sketch-based image retrieval is deep metric learning,
Our technique can be extended to a wide range of face-analysis applications including sketch-based \textit{face recognition}, \textit{generation}, etc.
% \textit{person re-identification}, as well as to other cross-modal retrieval tasks.
To the best of our knowledge, we are not aware of any particular limitation and negative societal impact of our proposed XModalViT framework, however, if our method is adopted for the aforementioned applications, care should be given to control privacy violation issues.

% \anjan{Do you think SBIR could have any negative societal impact? I don't think.}
% \anjan{It is not clear how this techniques could be applied to human faces? You can use the following texts: The underlying technique of FG-SBIR is deep metric learning. Deep metric learning can be applied to a wide range of applications including face recognition (FR), person re-identification (re-ID), as well as to other cross-modal retrieval tasks.} \anjan{privacy violation for FR and re-ID} For databases containing photos of human faces, fine-grained retrieval via query sketches is a useful functionality. If our method is adopted for such an application, the false-positive results may pose legal issues. The people whose faces are wrongly returned may not have provided the required consent for displaying their photos as a result of a false positive match.

% \anjan{I think this is not really a limitation. It's kind of the model capacity.} Fine-grained matching of details has an inherent issue for photo databases that contain a large number of visually similar classes, with subtle fine-grained similarities, but more abstract, category-level dissimilarities. Performing fine-grained retrieval from such databases may retrieve photos from a class, that although would have significant visual similarities with that of the query sketch, but may belong to a different category altogether. This could especially be a problem in scenarios where the photo database may have age-restricted content. Care should be taken while deploying a system based on our framework under such circumstances.

==> tex/08_app_backup.tex <==
\section*{Appendix}

\section{Further Experimental Details and Findings}
\subsection{Platform Details}
We implement our XModalViT model using the PyTorch \cite{Paszke2017PyTorch} deep learning framework, on an Ubuntu 20.04 workstation with a single Nvidia GeForce RTX 3090 GPU, an 8-core Intel Xeon processor and 32 GBs of RAM. Since we are using a fixed-size queue to store XMA representations, we do not have a dependency on batch-size for the purpose of negative sampling as part of our contrastive learning phase, which enables us to train both the teacher and the students on a single GPU. 

\subsection{Dataset Statistics}
    \begin{table}[!ht]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|c|c|c|c|c}
    Dataset & \#Classes & \#Photos & \#Sketches & \#Sketches/Photo & Test Fraction \\
    \hline
    QMUL-Shoe-V2 & -- & 2000 & 6648 & 2 to 4 & 0.1 \\
    QMUL-Chair-V2 & -- & 400 & 1275 & 2 to 4 & 0.1 \\
    \hline
    Sketchy & 125 & 12,500 & 75,471 & 5 to 9 & 0.1
    \end{tabular}
    }
    \caption{Details of the datasets used for experimental evaluation.}
    \label{tab:Datasets}
\end{table}

\subsection{Effects of Varying the Queue Sizes in XAQC}
We vary the XAQC queue sizes as $2^m$, where m $\in \{1,2,... \lfloor\log_2 N\rfloor\}$, and $N$ is the total number of datapoints. The observed trend has been graphically depicted in \cref{fig:queue_size_ablation}, where it can be seen that the accuracy is minimum at $m=1$, when the objective is equivalent to InfoNCE, which only performs reasonably with larger batch-sizes. However, the accuracy begins to saturate near its maximum at $m = \lfloor \log_2 N \rfloor$.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=4.5cm, height=3.5cm]{figures/quesz_acc1}
    \captionof{figure}{Acc@1 with varying XAQC queue sizes $2^m$, where m $\in \{1, 2, ...,\lfloor\log_2 N\rfloor\}$, and $N$ is the total number of datapoints.}
\label{fig:queue_size_ablation}
\end{figure}

\subsection{ViT+CNN Backbones}
While keeping the ViT-B teacher backbones, we switched the student backbones to ResNet18 \cite{He2016DeepRL} %with which 
and obtained acc@1 of 44.9\% and 63.21\% on the Shoe-V2 and Chair-V2 datasets respectively. %, using ViT-Base networks as the teacher encoders. 
However, with the Inception-v3 \cite{Szegedy2016Inceptionv3} network as the student backbones, the acc@1 on the same datasets drop to 42.5\% and 62.07\% respectively. This goes on to show that, once %the teacher 
our ViT-Base networks as the teacher encoders learn the fused cross-modal attention representations, the correct inductive biases in CNNs can be used to approximate them. However, for the teacher network, there is no straightforward way to formulate the XMA operator that would make sense over the space of CNN feature maps. The cross-modal interaction between the global class-token of one modality and the local patch embeddings of the other is something that can be more naturally defined for Vision Transformers.

\section{Pseudocodes}
This section provides algorithmic pseudocodes for the core components of the XModalViT framework.
\\[\baselineskip]
Notations like tuple assignment:
\begin{equation}
    (a, b) = (b, a)
\end{equation}
are inspired by Python's syntax.
The construct ``with no gradient" signifies that the output of the operation performed within the block is treated like a constant, and its computation does not affect the gradient of any of the learnable parameters that might have been used for that purpose.

\subsection{Modality Fusion Network}
% \IncMargin{1em}
\begin{algorithm}[!ht]
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}

\Input{A set of photos $\mathcal{P}$ and corresponding sketches $\mathcal{S}$; Cross-attention queue size $k$; Learning rate $\eta$; Number of epochs $N$}
\Output{Cross-Modal Fusion Network (Teacher): $\Gamma$}

$\mathcal{Q} \longleftarrow$ Randomly initialized queue of size $k$\\
\For{epoch $\leftarrow 1$ \KwTo $N$}{
    $p \sim \mathcal{P}, \; (s_1, s_2) \sim \mathcal{S} \; \mid \; p \xleftrightarrow{} (s_1, s_2)$\\
    
    $(\vectorname{x}^1_p, \vectorname{x}^1_s) \longleftarrow \Gamma(p, s_1)$ \\
    
    \tcp{Outputs are treated as constants}
    with no gradient: \\
     \Indp $(\vectorname{x}^2_p, \vectorname{x}^2_s) \longleftarrow \Gamma(p, s_2)$ \\
     \Indm
    
    $\mathcal{L}_{\text{teacher}} \longleftarrow \textbf{\texttt{XAQC}}(\vectorname{x}^1_p, \vectorname{x}^2_s, \mathcal{Q})$ \\
    
    $\mathcal{Q} \longleftarrow \mathcal{Q}$.enqueue$(\vectorname{x}^2_s)$\\
    $\Gamma \longleftarrow \Gamma - \eta \nabla_\Gamma \mathcal{L}_{\text{teacher}}$
}
\caption{\textsc{Modality-Fusion-Network}: Train the cross-modal attention (XMA) based teacher network, $\Gamma$, that fuses information across the photo and the sketch modalities.}
\label{alg:teacher}
\end{algorithm}

The objective of the \textsc{Modality-Fusion-Network} is to train the cross-modal attention (XMA) based teacher network, $\Gamma$, that fuses information across the photo and the sketch modalities. \Cref{alg:teacher} provides a pseudocode for the same.

$\mathcal{Q}$ is initialized as a queue of size $k$ containing random vectors, which is later used for storing XMA-sketch representations.
We sample a photo $p$ and 2 of its corresponding sketches $s_1$ and $s_2$. In line-5, $(p, s_1)$ is propagated through the teacher network for obtaining its XMA-photo embedding, $\vectorname{x}^1_p$. The XMA-sketch embedding, $\vectorname{x}^2_s$, for $(p, s_1)$ is computed in this manner. We then compute the XAQC loss for the teacher by treating $\vectorname{x}^2_s$ as a soft-target for $\vectorname{x}^1_p$ and all the representations in $\vectorname{x}^1_s$ as negatives. We then enqueue $\vectorname{x}^1_s$ into $\mathcal{Q}$ in line-9. We finally update the teacher network with the gradient of the XAQC loss with respect to its parameters.

\subsection{Cross-Modal Knowledge Distillation}

\begin{algorithm}[!ht]
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}

\Input{A set of photos $\mathcal{P}$ and corresponding sketches $\mathcal{S}$; Teacher network $\Gamma$; Cross-attention queue size $k$; Learning rate $\eta$; Number of epochs $N$}
\Output{Student Networks - Photo encoder $\xi_{\text{photo}}$ and sketch encoder $\xi_{\text{sketch}}$}

$\mathcal{Q}_\mathcal{P}, \mathcal{Q}_\mathcal{S} \longleftarrow$ Randomly initialized queues of size $k$\\
\For{epoch $\leftarrow 1$ \KwTo $N$}{
    $p_1 \sim \mathcal{P}, \; s_1 \sim \mathcal{S} \; \mid \; p_1 \xleftrightarrow{} s_1$ \\
    
    $p_2, p_3 \sim \mathcal{P}, \; s_2, s_3 \sim \mathcal{S} \; \mid \; p_2 \xleftrightarrow{} s_2, p_3 \xleftrightarrow{} s_3$ \\
    
    \tcp{Outputs are treated as constants}
    with no gradient: \\
        \For{$i \leftarrow 1$ \KwTo $3$}{
        $(\vectorname{x}_{p_i}, \vectorname{x}_{s_i}) \longleftarrow \Gamma(p_i, s_i)$ \\
        }
        % \Indm
    
    \For{$i \leftarrow 1$ \KwTo $3$}{
        $(\vectorname{z}_{p_i}, \vectorname{z}_{s_i}) \longleftarrow \xi_\text{photo}(p_i), \xi_\text{sketch}(s_i)$ \\
    }
    $\mathcal{L}^\text{photo-student}_\text{XAQC} \longleftarrow \textbf{\texttt{XAQC}}(\vectorname{x}_{p_1}, \vectorname{z}_{p_1}, \mathcal{Q}_\mathcal{P})$ \\
    
    $\mathcal{L}^\text{sketch-student}_\text{XAQC} \longleftarrow \textbf{\texttt{XAQC}}(\vectorname{x}_{s_1}, \vectorname{z}_{s_1}, \mathcal{Q}_\mathcal{S})$ \\
    
    $\mathcal{Q}_\mathcal{P} \longleftarrow \mathcal{Q}_\mathcal{P}$.enqueue$(\vectorname{x}_{p_1})$ \\
    $\mathcal{Q}_\mathcal{S} \longleftarrow \mathcal{Q}_\mathcal{S}$.enqueue$(\vectorname{x}_{s_1})$ \\
    
    \tcp{$m \in \{p, m\}$}
    $\pi^\text{teacher}_m \longleftarrow \psi_1(\vectorname{x}_{m_1}, \vectorname{x}_{m_2}) + \psi_2(\vectorname{x}_{m_1}, \vectorname{x}_{m_2}, \vectorname{x}_{m_3})$ \\
    $\pi^\text{student}_m \longleftarrow \psi_1(\vectorname{z}_{m_1}, \vectorname{z}_{m_2}) + \psi_2(\vectorname{z}_{m_1}, \vectorname{z}_{m_2}, \vectorname{z}_{m_3})$
    
    $\mathcal{L}_\text{XMRD} \longleftarrow
    \delta(\pi^\text{teacher}_p, \pi^\text{student}_p) + 
    \delta(\pi^\text{teacher}_s, \pi^\text{student}_s)$
    
    $\mathcal{L}_\text{student} \longleftarrow
    \mathcal{L}^\text{sketch-student}_\text{XAQC} + \mathcal{L}^\text{photo-student}_\text{XAQC} + \lambda \cdot \mathcal{L}_\text{XMRD}$

    $\xi_\text{photo} \longleftarrow \xi_\text{photo} - \nabla_{\xi_\text{photo}} \mathcal{L}_\text{student}$
    
    $\xi_\text{sketch} \longleftarrow \xi_\text{sketch} - \nabla_{\xi_\text{sketch}} \mathcal{L}_\text{student}$
}
\caption{\textsc{Cross-Modal-Knowledge-Distillation}: Decouple the domain of $\Gamma$ by transferring its representations to independent encoders, $\xi_\text{photo}$ and $\xi_\text{sketch}$.}
\label{alg:student}
\end{algorithm}

The objective of cross-modal knowledge distillation is to decouple the input-space of the modality fusion network (teacher), $\Gamma$, into independent, modality-specific encoders, $\xi_\text{photo}$ and $\xi_\text{sketch}$. \Cref{alg:student} describes the process in the form of a pseudocode.

We start by sampling 3 corresponding photo-sketch pairs $(p_1, s_1), (p_2, s_2)$ and $(p_3, s_3).$ We propagate these pairs through the modality fusion network (teacher), $\Gamma$, to obtain their XMA-photo and XMA-sketch embeddings. The photos and the sketches are then separately encoded via the photo and the sketch students respectively, to obtain the approximate versions of their XMA representations, \ie, $\vectorname{z}_{p_i}$ and $\vectorname{z}_{s_i}$. With the objective of aligning these $z_\mathlarger{*}$ representations with the true XMA representations, $x_\mathlarger{*}$, obtained from the teacher, we minimize the contrastive XAQC loss between the two (lines 11 and 12). We also aim to preserve the geometry of the teacher's representation space in that of the students' by distilling distance and angular relationships between arbitrary $k$-tuples of datapoints. This process of cross-modal relation distillation (XMRD) is depicted in lines 16-18. $m$, here, has been introduced for the purpose of conciseness, serving as an abstract notation for modality, \ie, standing for both photos and sketches. $\psi_1$ and $\psi_2$ are the distance and angle relation functions respectively, and $\delta$ is the Huber loss, as described in the main text. The total student loss is computed as the sum of the losses from the individual students and the XMRD loss (weighted by a balancing factor of $\lambda$). We finally update the individual students by the gradient of the total student loss with respect to the weights of the corresponding student encoders.

% \begin{figure*}[!t]
% \centering
% % \resizebox{\textwidth}{!}{
% \begin{tabular}{c}
% \includegraphics[width=0.71\textwidth]{umaps/shoev2_umap.png} \\
% \large{(a)} \\
% \includegraphics[width=0.71\textwidth]{umaps/chairv2_umap.png} \\
% \large{(b)} \\
% % \multicolumn{2}{c}{\includegraphics[width=\textwidth]{umaps/sketchy_umap.png}} \\
% \includegraphics[width=0.71\textwidth]{umaps/sketchy_umap.png} \\
% \large{(c)}
% % \multicolumn{2}{c}{\large{(c)}}
% \end{tabular}
% \caption{UMAP \cite{mcinnes2018umap-software} visualizations of photo-student (red) and sketch-student (blue) embeddings on the (a) QMUL-Shoe-V2 (b) QMUL-Chair-V2 and (c) Sketchy datasets.} \label{fig:umap_qmul}
% \end{figure*}

% \begin{figure*}[!ht]
% \centering
% \includegraphics[width=\textwidth]{umaps/sketchy_umap.png}
% \caption{UMAP \cite{mcinnes2018umap-software} visualization of photo-student (red) and sketch-student (blue) embeddings on Sketchy}
% \label{fig:umap_sketchy}
% \end{figure*}

\section{Embedding Visualizations}
\Cref{fig:umap_qmul} shows the test-set embeddings of the photo (red) and sketch (blue) student encoders, projected onto a 2-dimensional space via UMAP \cite{mcinnes2018umap-software}. The layout of the datapoints across the two modalities can be seen as being very similar, indicating that both the encoders have learned to model the distribution of the underlying shared abstract concept. As a result of this, and by the virtue of the instance-discriminative XAQC loss, photo-sketch pairs of the same instance get mapped close to each other, a phenomenon that has also been depicted in the visualizations.

\begin{figure}[!ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c}
\includegraphics[width=0.71\textwidth]{umaps/shoev2_umap.png} \\
\large{(a)} \\
\includegraphics[width=0.71\textwidth]{umaps/chairv2_umap.png} \\
\large{(b)} \\
\includegraphics[width=0.71\textwidth]{umaps/sketchy_umap.png} \\
\large{(c)}
\end{tabular}
}
\caption{UMAP \cite{mcinnes2018umap-software} visualizations of photo-student (red) and sketch-student (blue) embeddings on the (a) QMUL-Shoe-V2 (b) QMUL-Chair-V2 and (c) Sketchy datasets.} \label{fig:umap_qmul}
\end{figure}


% \setlength{\tabcolsep}{0pt}
% \renewcommand{\arraystretch}{1}
\begin{figure}[!ht]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c}
& & {\huge 1 \hspace{6pt}} & {\huge 2 \hspace{6pt}} & {\huge 3 \hspace{6pt}} & {\huge 4 \hspace{6pt}} & {\huge 5 \hspace{6pt}} & {\huge 6 \hspace{6pt}} & {\huge 7 \hspace{6pt}} & {\huge 8 \hspace{6pt}} & {\huge 9 \hspace{6pt}} & {\huge 10 \hspace{6pt}} \\
\raisebox{1.5cm}{\huge 1 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01772222_10951/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01772222_10951/0_n02176261_7522_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n01772222_10951/1_n01772222_10951_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01772222_10951/2_n02165105_3542_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01772222_10951/3_n02169497_6005_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01772222_10951/4_n01772222_5563_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01772222_10951/5_n01674464_377_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01772222_10951/6_n01498041_6780_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01772222_10951/7_n01772222_708_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01772222_10951/8_n01772222_5789_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01772222_10951/9_n01772222_11936_ph_0} \\ 
\raisebox{1.5cm}{\huge 2 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01877134_5530/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01877134_5530/0_n01877134_11906_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n01877134_5530/1_n01877134_5530_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01877134_5530/2_n03481172_11250_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01877134_5530/3_n02430045_4563_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01877134_5530/4_n02041246_9212_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01877134_5530/5_n01978930_9044_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01877134_5530/6_n02169497_2852_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01877134_5530/7_n04589593_13410_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01877134_5530/8_n01498041_10279_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01877134_5530/9_n02002724_2019_ph_0} \\ 
\raisebox{1.5cm}{\huge 3 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01887787_18038/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01887787_18038/0_n02503517_6624_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n01887787_18038/1_n01887787_18038_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01887787_18038/2_n01979526_2733_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01887787_18038/3_n01887787_923_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01887787_18038/4_n02503517_5117_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01887787_18038/5_n02391049_7851_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01887787_18038/6_n03028596_5115_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01887787_18038/7_n02391049_3220_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01887787_18038/8_n02411705_5029_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01887787_18038/9_n02391049_261_ph_0} \\ 
% \raisebox{1.5cm}{\huge 4 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01986214_24017/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01986214_24017/0_n01482330_7514_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01986214_24017/1_n02355227_14906_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01986214_24017/2_n02346627_7790_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01986214_24017/3_n01978930_9044_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01986214_24017/4_n02131653_5478_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n01986214_24017/5_n01986214_24017_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01986214_24017/6_n02076196_5323_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01986214_24017/7_n02106662_18922_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01986214_24017/8_n02068974_485_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n01986214_24017/9_n01664065_8823_ph_0} \\ 
\raisebox{1.5cm}{\huge 4 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02009912_732/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n02009912_732/0_n02009912_732_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02009912_732/1_n01791625_7354_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02009912_732/2_n02055803_338_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02009912_732/3_n01531178_5255_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02009912_732/4_n04128499_12318_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02009912_732/5_n02165105_2919_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02009912_732/6_n02483362_8084_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02009912_732/7_n02391994_12378_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02009912_732/8_n02391994_12378_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02009912_732/9_n02169497_7086_ph_0} \\ 
\raisebox{1.5cm}{\huge 5 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02121620_6042/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n02121620_6042/0_n02121620_6042_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02121620_6042/1_n02129165_3951_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02121620_6042/2_n01986214_1625_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02121620_6042/3_n12651611_7927_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02121620_6042/4_n01641391_10094_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02121620_6042/5_n02391994_18304_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02121620_6042/6_n02859184_7092_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02121620_6042/7_n02070430_7864_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02121620_6042/8_n04587648_3854_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02121620_6042/9_n04398044_15601_ph_0} \\ 
\raisebox{1.5cm}{\huge 6 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02167151_9858/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02167151_9858/0_n01772222_10890_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02167151_9858/1_n02168699_8557_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02167151_9858/2_n01772222_8692_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n02167151_9858/3_n02167151_9858_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02167151_9858/4_n02168699_6550_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02167151_9858/5_n02470325_9404_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02167151_9858/6_n11669921_25300_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02167151_9858/7_n02219486_7443_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02167151_9858/8_n02007558_8804_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02167151_9858/9_n02106662_13178_ph_0} \\ 
\raisebox{1.5cm}{\huge 7 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02206856_6708/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n02206856_6708/0_n02206856_6708_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02206856_6708/1_n01910747_11820_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02206856_6708/2_n01693334_3431_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02206856_6708/3_n09472597_21657_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02206856_6708/4_n03028596_5727_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02206856_6708/5_n03495258_8812_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02206856_6708/6_n09288635_14453_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02206856_6708/7_n02950826_33377_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02206856_6708/8_n02206856_1036_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02206856_6708/9_n02219486_23761_ph_0} \\ 
\raisebox{1.5cm}{\huge 8 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02219486_24977/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n02219486_24977/0_n02219486_24977_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02219486_24977/1_n02219486_5549_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02219486_24977/2_n02317335_779_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02219486_24977/3_n07695742_9181_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02219486_24977/4_n02764044_21188_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02219486_24977/5_n01697457_1191_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02219486_24977/6_n02129165_2015_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02219486_24977/7_n07753275_28771_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02219486_24977/8_n01697457_1463_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02219486_24977/9_n01944390_13160_ph_0} \\ 
\raisebox{1.5cm}{\huge 9 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02274259_15293/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n02274259_15293/0_n02274259_15293_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02274259_15293/1_n02274259_5703_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02274259_15293/2_n02895154_15087_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02274259_15293/3_n04389033_22507_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02274259_15293/4_n02958343_12509_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02274259_15293/5_n03930630_3476_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02274259_15293/6_n02274259_16258_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02274259_15293/7_n02834778_10158_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02274259_15293/8_n02169497_4717_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02274259_15293/9_n02391049_1789_ph_0} \\ 
\raisebox{1.5cm}{\huge 10 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02317335_18550/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n02317335_18550/0_n02317335_18550_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02317335_18550/1_n01496331_15801_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02317335_18550/2_n03633091_15372_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02317335_18550/3_n02317335_17188_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02317335_18550/4_n01944390_12478_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02317335_18550/5_n01663401_1069_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02317335_18550/6_n04373894_32946_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02317335_18550/7_n02605316_432_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02317335_18550/8_n01978930_9044_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02317335_18550/9_n04148054_2324_ph_0} \\ 
% \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/0_n02374451_1340_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/1_n02103406_5601_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/2_n02374451_2233_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/3_n02412080_7894_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/4_n04126066_10175_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/5_n02391994_14012_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/6_n03541923_4292_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/7_n03271574_1926_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/8_n03930630_5801_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/9_n01594787_14216_ph_0} \\ 
% \fontsize{1}{3}\selectfont 12 & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03452741_3792/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03452741_3792/0_n03452741_9020_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03452741_3792/1_n03452741_3792_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n03452741_3792/2_n03452741_3792_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03452741_3792/3_n03452741_15019_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03452741_3792/4_n03590841_11414_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03452741_3792/5_n07753592_6768_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03452741_3792/6_n04256520_33899_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03452741_3792/7_n03891251_312_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03452741_3792/8_n07753275_28771_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03452741_3792/9_n07697537_7480_ph_0} \\ 
% \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03633091_15277/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n03633091_15277/0_n03633091_15277_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03633091_15277/1_n04128499_2366_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03633091_15277/2_n04587404_18387_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03633091_15277/3_n02859184_7092_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03633091_15277/4_n01983481_10368_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03633091_15277/5_n01887787_1737_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03633091_15277/6_n02330245_8908_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03633091_15277/7_n02412080_6949_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03633091_15277/8_n04373894_37359_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03633091_15277/9_n01846331_11660_ph_0} \\ 
\raisebox{1.5cm}{\huge 11 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03790512_12399/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03790512_12399/0_n02834778_10391_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n03790512_12399/1_n03790512_12399_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03790512_12399/2_n02834778_10158_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03790512_12399/3_n07695742_11180_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03790512_12399/4_n03891251_7764_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03790512_12399/5_n07745940_2952_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03790512_12399/6_n02274259_16258_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03790512_12399/7_n03930630_3476_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03790512_12399/8_n07873807_4443_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n03790512_12399/9_n02958343_3671_ph_0} \\ 
\raisebox{1.5cm}{\huge 12 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n04589593_10706/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n04589593_10706/0_n04589593_10706_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n04589593_10706/1_n03227184_732_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n04589593_10706/2_n03222176_11276_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n04589593_10706/3_n03028079_31287_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n04589593_10706/4_n02676566_8467_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n04589593_10706/5_n03891251_728_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n04589593_10706/6_n07697313_8952_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n04589593_10706/7_n04589593_13289_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n04589593_10706/8_n03222318_8285_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n04589593_10706/9_n01816887_9978_ph_0} \\ 
% \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/0_n07695742_2935_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 4pt 4pt]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/1_n07695742_8726_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/2_n07697537_128_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/3_n07695742_8740_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/4_n07683786_25960_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/5_n07873807_2044_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/6_n07739125_7898_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/7_n07695742_8444_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/8_n07739125_3330_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/9_n01985128_13799_ph_0}
\end{tabular}}
\end{center}
\caption{Qualitative FG-SBIR results on Sketchy dataset.}
\label{fig:sketchy_long}
% : Apart from the instance-discriminative fine-grained features, the network learns attribute information such as classes with features that are closely related visually (rows 1, 3, 6, 11), object orientation and geometry (rows 8, 5, 4, 10), and even naturally occurring relationships (rows 5.1 and 5.2).}
\label{fig:qual_results_retrieval_results_app/Sketchy/}
\end{figure}






% \setlength{\tabcolsep}{0pt}
% \setlength{\tabcolsep}{0pt}
% \renewcommand{\arraystretch}{3}
\begin{figure}[!ht]
\begin{center}
\resizebox{\textwidth}{!}{
% \setlength\extrarowheight{-10pt}
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c}
\raisebox{1.5cm}{\huge 1 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2451386483/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ShoeV2//ShoeV2_2451386483/0_2451386483_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2451386483/1_3638376242_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2451386483/2_2478150015_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2451386483/3_4101385360_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2451386483/4_2540300078_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2451386483/5_2443085206_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2451386483/6_2450845009_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2451386483/7_2801452050_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2451386483/8_4756633009_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2451386483/9_2541991746_ph_0} \\ 
\raisebox{1.5cm}{\huge 2 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2487230450/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ShoeV2//ShoeV2_2487230450/0_2487230450_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2487230450/1_2478150015_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2487230450/2_2450845009_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2487230450/3_4101385360_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2487230450/4_4767160033_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2487230450/5_2552860271_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2487230450/6_2454505492_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2487230450/7_7261950344_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2487230450/8_4741285256_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2487230450/9_4764050012_ph_0} \\ 
\raisebox{1.5cm}{\huge 3 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2494561400/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ShoeV2//ShoeV2_2494561400/0_2494561400_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2494561400/1_4116545063_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2494561400/2_4338451008_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2494561400/3_7295185245_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2494561400/4_2545000078_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2494561400/5_4327011314_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2494561400/6_2482805404_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2494561400/7_4732075797_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2494561400/8_4751550012_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2494561400/9_2566485214_ph_0} \\ 
\raisebox{1.5cm}{\huge 4 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2495323065/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2495323065/0_2540300078_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ShoeV2//ShoeV2_2495323065/1_2495323065_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2495323065/2_2801452050_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2495323065/3_4732075797_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2495323065/4_4762060942_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2495323065/5_2465921927_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2495323065/6_4742785198_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2495323065/7_2547600078_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2495323065/8_2545000078_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2495323065/9_2534286052_ph_0} \\ 
\raisebox{1.5cm}{\huge 5 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2510850015/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ShoeV2//ShoeV2_2510850015/0_2510850015_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2510850015/1_2550685198_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2510850015/2_7246545614_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2510850015/3_2541991746_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2510850015/4_2484131533_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2510850015/5_7261950344_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2510850015/6_2482805404_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2510850015/7_2523200079_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2510850015/8_2478150015_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2510850015/9_7206900078_ph_0} \\ 
\raisebox{1.5cm}{\huge 6 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2517820640/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ShoeV2//ShoeV2_2517820640/0_2517820640_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2517820640/1_2529700078_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2517820640/2_7170422745_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2517820640/3_2548694437_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2517820640/4_2495323065_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2517820640/5_2507420408_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2517820640/6_2519323127_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2517820640/7_2534286052_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2517820640/8_2530845183_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2517820640/9_2530523163_ph_0} \\ 
\raisebox{1.5cm}{\huge 7 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521090008/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ShoeV2//ShoeV2_2521090008/0_2521090008_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521090008/1_4756633009_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521090008/2_2523200079_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521090008/3_4761100079_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521090008/4_2454505492_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521090008/5_2498760033_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521090008/6_2550551323_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521090008/7_2450845009_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521090008/8_2537401678_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521090008/9_2486900482_ph_0} \\ 
\raisebox{1.5cm}{\huge 8 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521600078/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ShoeV2//ShoeV2_2521600078/0_2521600078_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521600078/1_2534820062_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521600078/2_2486334191_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521600078/3_4726985835_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521600078/4_4747922797_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521600078/5_2812786508_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521600078/6_2549910060_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521600078/7_2741190211_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521600078/8_2529700078_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2521600078/9_2524500000_ph_0} \\ 
% \raisebox{1.5cm}{\huge 9 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2522901760/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ShoeV2//ShoeV2_2522901760/0_2522901760_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2522901760/1_2515245008_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2522901760/2_4742785198_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2522901760/3_2442786324_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2522901760/4_4307122902_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2522901760/5_2560200078_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2522901760/6_2777985908_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2522901760/7_2522831300_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2522901760/8_2454505492_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2522901760/9_2519205559_ph_0} \\ 
\raisebox{1.5cm}{\huge 9 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2524500000/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2524500000/0_2535745008_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2524500000/1_2560200078_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2524500000/2_2526910060_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2524500000/3_2519323127_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2524500000/4_2530523163_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2524500000/5_4104045897_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2524500000/6_2550821622_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2524500000/7_2576511599_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ShoeV2//ShoeV2_2524500000/8_2524500000_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2524500000/9_2449500078_ph_0} \\ 
\raisebox{1.5cm}{\huge 10 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2530845183/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ShoeV2//ShoeV2_2530845183/0_2530845183_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2530845183/1_2544020990_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2530845183/2_2517132593_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2530845183/3_7206900078_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2530845183/4_2507420408_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2530845183/5_2521820042_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2530845183/6_4328333962_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2530845183/7_2509212764_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2530845183/8_7223050344_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2530845183/9_7109520413_ph_0} \\ 
% \raisebox{1.5cm}{\huge 12 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2534820062/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ShoeV2//ShoeV2_2534820062/0_2534820062_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2534820062/1_4327011314_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2534820062/2_2750130450_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2534820062/3_2700230450_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2534820062/4_2529700078_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2534820062/5_2521190008_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2534820062/6_4340445835_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2534820062/7_2548694437_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2534820062/8_2484131533_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2534820062/9_4100832366_ph_0} \\ 
\raisebox{1.5cm}{\huge 11 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2542911599/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ShoeV2//ShoeV2_2542911599/0_2542911599_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2542911599/1_2517820640_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2542911599/2_4307122902_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2542911599/3_2520930792_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2542911599/4_2812520053_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2542911599/5_2478150015_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2542911599/6_2530845183_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2542911599/7_4762060942_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2542911599/8_2555700079_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2542911599/9_2572290035_ph_0} \\ 
\raisebox{1.5cm}{\huge 12 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2700230450/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ShoeV2//ShoeV2_2700230450/0_2700230450_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2700230450/1_2750130450_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2700230450/2_2787560000_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2700230450/3_2521190008_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2700230450/4_2550821622_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2700230450/5_2741190211_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2700230450/6_2537023178_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2700230450/7_2437921927_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2700230450/8_2548694437_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2700230450/9_7495445008_ph_0} \\ 
% \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2750130450/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ShoeV2//ShoeV2_2750130450/0_2750130450_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2750130450/1_2700230450_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2750130450/2_2550685198_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2750130450/3_4741045811_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2750130450/4_2521190008_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2750130450/5_2550821622_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2750130450/6_2494561400_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2750130450/7_2537023178_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2750130450/8_4100832366_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ShoeV2//ShoeV2_2750130450/9_2437700078_ph_0} \\ 
\end{tabular}
}\end{center}
\caption{Qualitative FG-SBIR results on Shoe-V2 dataset.}
\label{fig:shoe_v2_long}
% : Most instances with a sufficient number of fine-grained instance-discriminative features can be seen to appear in the top 1. However, for the ones that do get demoted in rank, (row 4), are preceded by an instance that have noticeable features in common that could cause confusion. Some false positive top-1 results might occur as a side-effect of modality fusion (row 10), where the embedding space also captures the texture information from the photo modality, which may not always be necessarily relevant (causing a shoe with a similar shiny texture as the ground-truth being returned as the first retrieval result in row 10).}
\label{fig:qual_results_retrieval_results_app/ShoeV2/}
\end{figure}



% \renewcommand{\arraystretch}{3}
\begin{figure*}[!ht]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c}
\raisebox{1.5cm}{\huge 1 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_6125-61003/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ChairV2//ChairV2_6125-61003/0_6125-61003_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_6125-61003/1_5840-44_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_6125-61003/2_0527-blanc_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_6125-61003/3_5788521_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_6125-61003/4_70288036_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_6125-61003/5_gu-026495_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_6125-61003/6_70238188_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_6125-61003/7_70311904_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_6125-61003/8_60282191_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_6125-61003/9_ma3-050_ph_0} \\ 
\raisebox{1.5cm}{\huge 2 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_00332250_v1/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ChairV2//ChairV2_00332250_v1/0_00332250_v1_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_00332250_v1/1_10267046_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_00332250_v1/2_3110-3438-leawalnu_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_00332250_v1/3_SOFJNH136YEL-UK_v1_Sul_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_00332250_v1/4_CHAMLY005RED-UK_v1_Ras_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_00332250_v1/5_300-030-031_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_00332250_v1/6_49900952_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_00332250_v1/7_SOFLULU15ORA-UK_v1_ChateletOran_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_00332250_v1/8_sd12-o_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_00332250_v1/9_70311904_v1_ph_0} \\ 
\raisebox{1.5cm}{\huge 3 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_4596352_v1_Brown/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ChairV2//ChairV2_4596352_v1_Brown/0_4596352_v1_Brown_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_4596352_v1_Brown/1_39122449_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_4596352_v1_Brown/2_6179296_v1_Black_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_4596352_v1_Brown/3_mosmkedb_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_4596352_v1_Brown/4_40320957_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_4596352_v1_Brown/5_4834052_v1_White_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_4596352_v1_Brown/6_6173656_v1_Blue_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_4596352_v1_Brown/7_6917025_v1_Chocolate_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_4596352_v1_Brown/8_cm1129-rnrn-lbne_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_4596352_v1_Brown/9_90290463_v1_ph_0} \\ 
\raisebox{1.5cm}{\huge 4 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_5788521/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ChairV2//ChairV2_5788521/0_5788521_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_5788521/1_sdasg046-f5_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_5788521/2_m0140101_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_5788521/3_9106000-017_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_5788521/4_70238188_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_5788521/5_4897-b4_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_5788521/6_2287-rouge_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_5788521/7_6125-61003_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_5788521/8_gu-026495_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_5788521/9_10118lem-662-ver_ph_0} \\ 
\raisebox{1.5cm}{\huge 5 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_10267046_v1/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ChairV2//ChairV2_10267046_v1/0_10267046_v1_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_10267046_v1/1_60282191_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_10267046_v1/2_20312010_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_10267046_v1/3_SOFJNH136YEL-UK_v1_Sul_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_10267046_v1/4_2287-rouge_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_10267046_v1/5_70311904_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_10267046_v1/6_300-030-031_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_10267046_v1/7_49900952_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_10267046_v1/8_3110-3438-leawalnu_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_10267046_v1/9_9106000-017_ph_0} \\ 
\raisebox{1.5cm}{\huge 6 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30299027_v1/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30299027_v1/0_CHALEON02GRY-UK_v1_MinkGrey_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30299027_v1/1_CHAFLN017GRY-UK_v1_PersianGrey_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30299027_v1/2_6917025_v1_Chocolate_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ChairV2//ChairV2_30299027_v1/3_30299027_v1_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30299027_v1/4_sco_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30299027_v1/5_SOFCOS001GRY-UK_v1_Pe_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30299027_v1/6_3325720_v1_Natural_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30299027_v1/7_5482032_v1_Chocolate_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30299027_v1/8_CHAQTI006GRY-UK_v1_UrbanGrey_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30299027_v1/9_4123361_v1_Chocolate_ph_0} \\ 
\raisebox{1.5cm}{\huge 7 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30308569_v1/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30308569_v1/0_5788521_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ChairV2//ChairV2_30308569_v1/1_30308569_v1_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30308569_v1/2_222021-1201603hal130_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30308569_v1/3_sdasg046-f5_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30308569_v1/4_10118lem-662-ver_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30308569_v1/5_4897-b4_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30308569_v1/6_50311957_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30308569_v1/7_slasg046-laque-noir_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30308569_v1/8_20153-muu_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_30308569_v1/9_6155-64009_ph_0} \\ 
\raisebox{1.5cm}{\huge 8 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40209615_v1/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ChairV2//ChairV2_40209615_v1/0_40209615_v1_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40209615_v1/1_6917025_v1_Chocolate_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40209615_v1/2_mgup-_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40209615_v1/3_CHAQTI006GRY-UK_v1_UrbanGrey_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40209615_v1/4_90095428_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40209615_v1/5_CHAFLN017GRY-UK_v1_PersianGrey_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40209615_v1/6_mosmkedb_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40209615_v1/7_70238188_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40209615_v1/8_90174642_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40209615_v1/9_CHALEON02GRY-UK_v1_MinkGrey_ph_0} \\ 
\raisebox{1.5cm}{\huge 9 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40320957_v1/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ChairV2//ChairV2_40320957_v1/0_40320957_v1_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40320957_v1/1_520-030-018_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40320957_v1/2_30308569_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40320957_v1/3_80273096_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40320957_v1/4_20320958_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40320957_v1/5_4596352_v1_Brown_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40320957_v1/6_7010400_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40320957_v1/7_6179296_v1_Black_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40320957_v1/8_CHABDL002BLU-UK_v1_ThamesBlue_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_40320957_v1/9_70288036_v1_ph_0} \\ 
% \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_70311904_v1/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_70311904_v1/0_00332250_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_70311904_v1/1_49900952_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_70311904_v1/2_20312010_v1_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ChairV2//ChairV2_70311904_v1/3_70311904_v1_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_70311904_v1/4_SOFJNH136YEL-UK_v1_Sul_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_70311904_v1/5_CHAMLY005RED-UK_v1_Ras_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_70311904_v1/6_3110-3438-leawalnu_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_70311904_v1/7_10259485_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_70311904_v1/8_5840-44_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_70311904_v1/9_9106000-017_ph_0} \\ 
\raisebox{1.5cm}{\huge 10 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_CHAMLY005RED-UK_v1_Ras/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_CHAMLY005RED-UK_v1_Ras/0_CHAFLN017GRY-UK_v1_PersianGrey_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ChairV2//ChairV2_CHAMLY005RED-UK_v1_Ras/1_CHAMLY005RED-UK_v1_Ras_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_CHAMLY005RED-UK_v1_Ras/2_CHAQTI006GRY-UK_v1_UrbanGrey_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_CHAMLY005RED-UK_v1_Ras/3_09090464_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_CHAMLY005RED-UK_v1_Ras/4_CHALEON02GRY-UK_v1_MinkGrey_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_CHAMLY005RED-UK_v1_Ras/5_CHAPRO002YEL-UK_v1_AmberLinen_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_CHAMLY005RED-UK_v1_Ras/6_SOFJNH136YEL-UK_v1_Sul_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_CHAMLY005RED-UK_v1_Ras/7_70238188_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_CHAMLY005RED-UK_v1_Ras/8_70311904_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_CHAMLY005RED-UK_v1_Ras/9_4123361_v1_Chocolate_ph_0} \\ 
\raisebox{1.5cm}{\huge 11 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_cm8706-rnrn/0_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ChairV2//ChairV2_cm8706-rnrn/0_cm8706-rnrn_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_cm8706-rnrn/1_222021-1201603hal130_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_cm8706-rnrn/2_f054110-022_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_cm8706-rnrn/3_4826792_v1_Charcoal_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_cm8706-rnrn/4_6155-64009_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_cm8706-rnrn/5_19127810_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_cm8706-rnrn/6_10259485_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_cm8706-rnrn/7_cm1129-rnrn-lbne_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_cm8706-rnrn/8_4897-b4_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_cm8706-rnrn/9_CHALOTU04GRY-UK_v1_SilverGrey_ph_0} \\ 
% \raisebox{1.5cm}{\huge 12 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_f056103-022-41/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_f056103-022-41/0_222021-1201603hal130_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ChairV2//ChairV2_f056103-022-41/1_f056103-022-41_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_f056103-022-41/2_mosnu_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_f056103-022-41/3_f054110-022_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_f056103-022-41/4_00332250_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_f056103-022-41/5_90290463_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_f056103-022-41/6_50321433_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_f056103-022-41/7_20153-muu_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_f056103-022-41/8_812055-1009000_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_f056103-022-41/9_0527-blanc_ph_0} \\ 
\raisebox{1.5cm}{\huge 12 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_gouvy45-o/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_gouvy45-o/0_60240035_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_gouvy45-o/1_10118lem-662-ver_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ChairV2//ChairV2_gouvy45-o/2_gouvy45-o_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_gouvy45-o/3_620080pp4097_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_gouvy45-o/4_80273096_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_gouvy45-o/5_2287-rouge_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_gouvy45-o/6_302016130043_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_gouvy45-o/7_12010721051_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_gouvy45-o/8_60282191_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_gouvy45-o/9_90290463_v1_ph_0} \\ 
% \raisebox{1.5cm}{\huge 14 \hspace{6pt}} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_ma3-050/0_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_ma3-050/0_70311904_v1_ph_0} & \includegraphics[width=3cm, height=3cm, cfbox=ForestGreen 2pt 2pt]{retrieval_results_app/ChairV2//ChairV2_ma3-050/1_ma3-050_ph_1} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_ma3-050/2_12010721051_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_ma3-050/3_gu-026495_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_ma3-050/4_60240035_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_ma3-050/5_90095428_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_ma3-050/6_520-030-018_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_ma3-050/7_00332250_v1_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_ma3-050/8_300-030-031_ph_0} & \includegraphics[width=3cm, height=3cm]{retrieval_results_app/ChairV2//ChairV2_ma3-050/9_2287-rouge_ph_0} \\ 
\end{tabular}
}\end{center}
\caption{Qualitative FG-SBIR results on Chair-V2 dataset.}
\label{fig:chair_v2_long}
% : The modality fusion operator is able to capture cross-modal information such as color and texture, which are beyond the geometric structure of sketches (rows 4, 5, 7), while being able to able to attend to the modality-native attributes, such as structural geometry and orientation (rows 3, 8, 9, 10, 11).}
\label{fig:qual_results_retrieval_results_app/ChairV2/}
\end{figure*}


\section{Qualitative Results}

\subsection{Sketchy Dataset}
Apart from the instance-discriminative fine-grained features, the network learns attribute information such as classes with features that are closely related visually (rows 1, 3, 6, 11 of \cref{fig:sketchy_long}), object orientation and geometry (rows 8, 5, 4, 10 \cref{fig:sketchy_long}), and even naturally occurring relationships (rows 5.1 and 5.2 \cref{fig:sketchy_long}).

\subsection{QMUL-Shoe-V2 Dataset}
Most  instances  with  a  sufficient  number  of  fine-grained  instance-discriminative features can be seen to appear in the top 1.  However, for the ones that do get demoted in rank, (row 4 of \cref{fig:shoe_v2_long}), are preceded by an instance that have noticeable features in common that could cause confusion. Some false positive top-1 results might occur as a side-effect of modality fusion (row 10 of \cref{fig:shoe_v2_long}), where the embedding space also captures the texture information from the photo modality, which may not always be necessarily relevant (causing a shoe with a similar shiny texture as the ground-truth being returned as the first retrieval result in row 10 of \cref{fig:shoe_v2_long}).

\subsection{QMUL-Chair-V2 Dataset}
The modality fusion operator is able to capture cross-modal information such as color and texture, which are beyond the geometric structure of sketches (rows 4, 5, 7 of \cref{fig:chair_v2_long}), while being able to able to attend to the modality-native attributes, such as structural geometry and orientation (rows 3, 8, 9, 10, 11 of \cref{fig:chair_v2_long}).


==> tex/combined_qualitative_results.tex <==
\begin{figure*}[t]
\begin{minipage}{0.76\textwidth}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c}
\includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/s/0_0} & \includegraphics[width=0.5cm, height=0.5cm, cfbox=ForestGreen 1pt 1pt]{retrieval_results/s/0_s_ph_1} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/s/1_4875815_v1_Cream_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/s/2_saku231-vi30_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/s/3_sd1854-1754c_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/s/4_923-b_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/s/5_m_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/s/6_8810-4N_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/s/7_mc4-s_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/s/8_f056104-44bl-s042_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/s/9_juju-_ph_0} \\ 
\includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/09048031_v1/0_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/09048031_v1/0_50267049_v1_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/09048031_v1/1_69028836_v1_ph_0} & \includegraphics[width=0.5cm, height=0.5cm, cfbox=ForestGreen 1pt 1pt]{retrieval_results/09048031_v1/2_09048031_v1_ph_1} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/09048031_v1/3_SOFSTT003BRO-UK_v1_OxfordBrownPremiumLeather_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/09048031_v1/4_10205181_v1_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/09048031_v1/5_20204925_v1_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/09048031_v1/6_70217652_v1_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/09048031_v1/7_CHAHDX003BRO-UK_v1_SaddleBrownPremiumLeather_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/09048031_v1/8_8620821_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/09048031_v1/9_10240575_v1_ph_0} \\ 
\includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/9855070/0_0} & \includegraphics[width=0.5cm, height=0.5cm, cfbox=ForestGreen 1pt 1pt]{retrieval_results/9855070/0_9855070_ph_1} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/9855070/1_40307951_v1_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/9855070/2_90305775_v1_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/9855070/3_40044196_v1_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/9855070/4_10208537_v1_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/9855070/5_10295902_v1_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/9855070/6_70288630_v1_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/9855070/7_80275340_v1_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/9855070/8_80208529_v1_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/9855070/9_70321432_v1_ph_0} \\
\includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2490834202/0_0} & \includegraphics[width=0.5cm, height=0.5cm, cfbox=ForestGreen 1pt 1pt]{retrieval_results/ShoeV2_2490834202/0_2490834202_ph_1} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2490834202/1_2360634005_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2490834202/2_1226293036_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2490834202/3_1876794090_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2490834202/4_1988900482_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2490834202/5_1667230450_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2490834202/6_1683504535_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2490834202/7_1433503718_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2490834202/8_1952585019_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2490834202/9_1968094213_ph_0} \\ 
\includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2269900078/0_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2269900078/0_1823902757_ph_0} & \includegraphics[width=0.5cm, height=0.5cm, cfbox=ForestGreen 1pt 1pt]{retrieval_results/ShoeV2_2269900078/1_2269900078_ph_1} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2269900078/2_2286000078_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2269900078/3_1832104493_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2269900078/4_1880222624_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2269900078/5_1381500078_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2269900078/6_1896300078_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2269900078/7_1605500078_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2269900078/8_2241045008_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_2269900078/9_2186100079_ph_0} \\ 
\includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_1944150015/0_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_1944150015/0_2242561028_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_1944150015/1_1956700078_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_1944150015/2_1503800078_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_1944150015/3_1812800078_ph_0} & \includegraphics[width=0.5cm, height=0.5cm, cfbox=ForestGreen 1pt 1pt]{retrieval_results/ShoeV2_1944150015/4_1944150015_ph_1} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_1944150015/5_1416400078_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_1944150015/6_2384850012_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_1944150015/7_2402600079_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_1944150015/8_2288065281_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results/ShoeV2_1944150015/9_1852145724_ph_0}
\end{tabular}}
\vspace{-10pt}
\caption{Qualitative retrieval results of our method for fine-grained SBIR on the QMUL Shoe-V2 and QMUL Chair-V2 datasets}
\label{fig:qual_results_retrieval_results}
\end{minipage}%
\hspace{0.02\textwidth}%
\begin{minipage}{0.22\textwidth}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}c}
\includegraphics[width=7cm]{attention_maps/SG74_3.png} \\
\includegraphics[width=7cm]{attention_maps/s51vs_8.png} \\
\includegraphics[width=7cm]{attention_maps/s51vs_9.png} \\
\includegraphics[width=7cm]{attention_maps/CHALULU08ORA-UK_v1_ChateletOran_1.png} \\
\includegraphics[width=7cm]{attention_maps/CHALULU08ORA-UK_v1_ChateletOran_4.png} \\
\includegraphics[width=7cm]{attention_maps/923-b_9.png}
\end{tabular}}
\vspace{-10pt}
\caption{Attention maps on photos and corresponding sketches obtained from the student encoders.}
\label{AttentionMaps}
\end{minipage}
\end{figure*}
\vspace{-10pt}

==> tex/combined_qualitative_results2.tex <==
{
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{0.5}
\begin{figure*}[t]
\begin{minipage}{0.78\textwidth}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c}
\includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2550685198/0_0} & \includegraphics[width=0.5cm, height=0.5cm, cfbox=ForestGreen 1pt 1pt]{retrieval_results2/ShoeV2_2550685198/0_2550685198_ph_1} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2550685198/1_2550451459_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2550685198/2_4314005229_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2550685198/3_7246545614_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2550685198/4_7206900078_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2550685198/5_2510850015_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2550685198/6_2543620104_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2550685198/7_2541761400_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2550685198/8_2507705526_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2550685198/9_2544020990_ph_0} \\ 
% \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2787660000/0_0} & \includegraphics[width=0.5cm, height=0.5cm, cfbox=ForestGreen 1pt 1pt]{retrieval_results2/ShoeV2_2787660000/0_2787660000_ph_1} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2787660000/1_2534965087_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2787660000/2_2708234163_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2787660000/3_2542300079_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2787660000/4_2548694437_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2787660000/5_4327011314_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2787660000/6_2537401678_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2787660000/7_4116545063_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2787660000/8_2494561400_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2787660000/9_4731791453_ph_0} \\ 
\includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2549910060/0_0} & \includegraphics[width=0.5cm, height=0.5cm, cfbox=ForestGreen 1pt 1pt]{retrieval_results2/ShoeV2_2549910060/0_2549910060_ph_1} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2549910060/1_2520930792_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2549910060/2_2557411599_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2549910060/3_2555700079_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2549910060/4_7162350344_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2549910060/5_2508445009_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2549910060/6_4321712270_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2549910060/7_2454505492_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2549910060/8_2534586529_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ShoeV2_2549910060/9_2517900000_ph_0} \\ 
\includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_slasg046-laque-noir/0_0} & \includegraphics[width=0.5cm, height=0.5cm, cfbox=ForestGreen 1pt 1pt]{retrieval_results2/ChairV2_slasg046-laque-noir/0_slasg046-laque-noir_ph_1} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_slasg046-laque-noir/1_sdasg046-f5_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_slasg046-laque-noir/2_30308569_v1_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_slasg046-laque-noir/3_CHALEON02GRY-UK_v1_MinkGrey_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_slasg046-laque-noir/4_4897-b4_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_slasg046-laque-noir/5_300-030-031_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_slasg046-laque-noir/6_60282191_v1_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_slasg046-laque-noir/7_STLBERG11GRY-UK_v1_StonewithContrastPi_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_slasg046-laque-noir/8_10118lem-662-ver_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_slasg046-laque-noir/9_CHAPRO002YEL-UK_v1_AmberLinen_ph_0} \\ 
\includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_cm8706-rnrn/0_0} & \includegraphics[width=0.5cm, height=0.5cm, cfbox=ForestGreen 1pt 1pt]{retrieval_results2/ChairV2_cm8706-rnrn/0_cm8706-rnrn_ph_1} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_cm8706-rnrn/1_6155-64009_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_cm8706-rnrn/2_f054110-022_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_cm8706-rnrn/3_4826792_v1_Charcoal_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_cm8706-rnrn/4_CHABDL002BLU-UK_v1_ThamesBlue_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_cm8706-rnrn/5_mosmkedb_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_cm8706-rnrn/6_812055-1009000_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_cm8706-rnrn/7_19127810_v1_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_cm8706-rnrn/8_222021-1201603hal130_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_cm8706-rnrn/9_6159-61003_ph_0} \\ 
% \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_4826792_v1_Charcoal/0_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_4826792_v1_Charcoal/0_222021-1201603hal130_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_4826792_v1_Charcoal/1_cm8706-rnrn_ph_0} & \includegraphics[width=0.5cm, height=0.5cm, cfbox=ForestGreen 1pt 1pt]{retrieval_results2/ChairV2_4826792_v1_Charcoal/2_4826792_v1_Charcoal_ph_1} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_4826792_v1_Charcoal/3_6155-64009_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_4826792_v1_Charcoal/4_20153-muu_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_4826792_v1_Charcoal/5_CHABDL002BLU-UK_v1_ThamesBlue_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_4826792_v1_Charcoal/6_CHALOTU04GRY-UK_v1_SilverGrey_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_4826792_v1_Charcoal/7_cm1129-rnrn-lbne_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_4826792_v1_Charcoal/8_mosmkedb_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results2/ChairV2_4826792_v1_Charcoal/9_f054110-022_ph_0} \\
\includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/0_0} & \includegraphics[width=0.5cm, height=0.5cm, cfbox=ForestGreen 1pt 1pt]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/0_n02374451_1340_ph_1} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/1_n02103406_5601_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/2_n02374451_2233_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/3_n02412080_7894_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/4_n04126066_10175_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/5_n02391994_14012_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/6_n03541923_4292_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/7_n03271574_1926_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/8_n03930630_5801_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n02374451_1340/9_n01594787_14216_ph_0} \\ 
\includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/0_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/0_n07695742_2935_ph_0} & \includegraphics[width=0.5cm, height=0.5cm, cfbox=ForestGreen 1pt 1pt]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/1_n07695742_8726_ph_1} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/2_n07697537_128_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/3_n07695742_8740_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/4_n07683786_25960_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/5_n07873807_2044_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/6_n07739125_7898_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/7_n07695742_8444_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/8_n07739125_3330_ph_0} & \includegraphics[width=0.5cm, height=0.5cm]{retrieval_results_app/Sketchy//Sketchy_n07695742_8726/9_n01985128_13799_ph_0} \\
\end{tabular}}
\caption{Qualitative FG-SBIR results of our method on the Shoe-V2, Chair-V2 and Sketchy datasets. \massi{I would enlarge Fig. 4 and rotate horizontally Fig5 (adding more examples if possible and even with baseline CAMs if we have them). At the moment Fig. 5 is quite squeezed and might be hard to read/see its content}}
% \caption{Qualitative retrieval results of our method for FG-SBIR on the Shoe-V2, Chair-V2 and Sketchy datasets.}
% \massi{we may add qualitatives also on Sketchy (either here or in the suppmat)} \anjan{Yes, I think we can add them in the supplementary material.}
\label{fig:qual_results_retrieval_results}
\end{minipage}%
\hspace{0.0\textwidth}%
\begin{minipage}{0.215\textwidth}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}c}
% \includegraphics[width=7cm]{attention_maps2/shoe/7495445008_8.png} \\
% \includegraphics[width=7cm]{attention_maps2/shoe/2534820062_16.png} \\
% \includegraphics[width=7cm]{attention_maps2/shoe/2547600078_19.png} \\
% \includegraphics[width=7cm]{attention_maps2/chair/222021-1201603hal130_0.png} \\
% \includegraphics[width=7cm]{attention_maps2/chair/4897-b4_16.png} \\
% \includegraphics[width=7cm]{attention_maps2/chair/10111-marcel_8.png}

\includegraphics[width=7cm]{attention_maps3/shoe/2550685198_16.png} \\
\includegraphics[width=7cm]{attention_maps3/shoe/2521190008_16.png} \\
\includegraphics[width=7cm]{attention_maps3/chair/3257867_v1_Natural_16.png} \\
\includegraphics[width=7cm]{attention_maps3/chair/10111-marcel_10.png} \\
\includegraphics[width=7cm]{attention_maps3/sketchy/n01641391_7089_3.png} \\
\includegraphics[width=7cm]{attention_maps3/sketchy/n09472597_35497_1.png}


% \includegraphics[width=7cm]{attention_maps/s51vs_8.png} \\
% \includegraphics[width=7cm]{attention_maps/s51vs_9.png} \\
% \includegraphics[width=7cm]{attention_maps/CHALULU08ORA-UK_v1_ChateletOran_1.png} \\
% \includegraphics[width=7cm]{attention_maps/CHALULU08ORA-UK_v1_ChateletOran_4.png} \\
% \includegraphics[width=7cm]{attention_maps/923-b_9.png}
\end{tabular}}
\caption{Attention maps on photos and corresponding sketches obtained from the student encoders. }
\label{AttentionMaps}
\end{minipage}
\end{figure*}
}
